Universal flux-based control of a $\pi$-SQUID

We describe a protocol for the universal control of non-ideal $\pi$-periodic superconducting qubits. Our proposal relies on a $\pi$-SQUID: a superconducting loop formed by two $\pi$-periodic circuit elements, with an external magnetic flux threading the circuit. The system exhibits an extensive sweet spot around half-flux where residual $2\pi$-periodic Cooper pair tunneling is highly suppressed. We demonstrate that universal single-qubit operations can be realised by tuning the flux adiabatically and diabatically within this broad sweet spot. We also assess how residual $2\pi$-periodicity in $\pi$-SQUIDs impacts holonomic phase gates.

==> figures/circuits.tex <==
%%%%%%%%%%%%%%%%%%%%%%
%% Circuit elements %%
%%%%%%%%%%%%%%%%%%%%%%

\colorlet{Background}{white}
\colorlet{WireColor}{black}

\newcommand\WireBuffer{1}
\newcommand\WireSpacing{0.75}
\newcommand\WireLinewidth{1.25}
\newcommand\WireCorners{5}

%%%%%%%%%%%%%%%
%% Capacitor %%

\newcommand\CapLength{1}
\newcommand\CapWidth{0.1}
\newcommand\CapSpacing{0.15}

\def\Capacitor#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \draw [line width=\WireLinewidth, color=Background, fill=Background, rounded corners=2] 
        (\CapSpacing/2, \CapLength/2) rectangle (-\CapSpacing/2, -\CapLength/2);
    \draw [line width=\WireLinewidth, color=WireColor, fill=WireColor, rounded corners=1] 
        (-\CapSpacing/2, -\CapLength/2) rectangle (-\CapSpacing/2 - \CapWidth, \CapLength/2);
    \draw [line width=\WireLinewidth, color=WireColor, fill=WireColor, rounded corners=1] 
        (\CapSpacing/2, -\CapLength/2) rectangle (\CapSpacing/2 + \CapWidth, \CapLength/2);
\end{scope}
}

%%%%%%%%%%%%%%
%% Inductor %%

\newcommand\IndLength{1}
\newcommand\IndWidth{0.4}
\newcommand\IndDistanceLong{3.5}
\newcommand\IndDistanceShort{2}

\def\Inductor#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \draw [line width=\WireLinewidth, color=WireColor, fill=Background, rounded corners=5] 
        (0, -\IndLength/2) to [out=180, in=-90, distance=\IndDistanceShort] 
        (-\IndWidth/2, -3*\IndLength/8) to [out=90, in=90, distance=\IndDistanceLong] 
        (+\IndWidth/2, -\IndLength/4) to [out=-90, in=-90, distance=\IndDistanceLong] 
        (-\IndWidth/2, -\IndLength/8) to [out=90, in=90, distance=\IndDistanceLong] 
        (+\IndWidth/2, 0) to [out=-90, in=-90, distance=\IndDistanceLong] 
        (-\IndWidth/2, \IndLength/8) to [out=90, in=90, distance=\IndDistanceLong] 
        (+\IndWidth/2, \IndLength/4) to [out=-90, in=-90, distance=\IndDistanceLong]
        (-\IndWidth/2, 3*\IndLength/8) to [out=90, in=180, distance=\IndDistanceShort] 
        (0, \IndLength/2);
\end{scope}
}

%%%%%%%%%%%%%%%%%%%%%%%%
%% Josephson junction %%

\newcommand\JJWidth{0.5}

\def\JJunction#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \draw [line width=\WireLinewidth, color=WireColor, fill=Background, rounded corners=2] 
        (-\JJWidth/2, -\JJWidth/2) rectangle (\JJWidth/2, \JJWidth/2);
    \clip [rounded corners=2] 
        (-\JJWidth/2, -\JJWidth/2) rectangle (\JJWidth/2, \JJWidth/2);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (-\JJWidth/2, -\JJWidth/2) to (\JJWidth/2, \JJWidth/2);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (-\JJWidth/2, \JJWidth/2) to (\JJWidth/2, -\JJWidth/2);
\end{scope}
}

\def\JJunctionIdeal#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \clip [rounded corners=2] 
        (-\JJWidth/2, -\JJWidth/2) rectangle (\JJWidth/2, \JJWidth/2);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (-\JJWidth/2, -\JJWidth/2) to (\JJWidth/2, \JJWidth/2);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (-\JJWidth/2, \JJWidth/2) to (\JJWidth/2, -\JJWidth/2);
\end{scope}
}

%%%%%%%%%%%%%%%%%
%% Pi junction %%

\newcommand\PJWidth{\JJWidth}

\def\PJunction#1#2{
\begin{scope}[shift={#1}, rotate=(45+#2)]
    \draw [line width=\WireLinewidth, color=WireColor, fill=Background, rounded corners=2] 
        (-\PJWidth/2, -\PJWidth/2) rectangle (\PJWidth/2, \PJWidth/2);
    \clip [rounded corners=2] 
        (-\PJWidth/2, -\PJWidth/2) rectangle (\PJWidth/2, \PJWidth/2);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (0, -\PJWidth/2) to (0, \PJWidth/2);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (-\PJWidth/2, 0) to (\PJWidth/2, 0);
\end{scope}
}

\def\PJunctionIdeal#1#2{
\begin{scope}[shift={#1}, rotate=(45+#2)]
    \draw [line width=\WireLinewidth, color=WireColor, fill=Background, rounded corners=2] 
        (-\PJWidth/2, -\PJWidth/2) rectangle (\PJWidth/2, \PJWidth/2);
\end{scope}
}

%%%%%%%%%%%%
%% Ground %%

\newcommand\GroundWidth{0.6}
\newcommand\GroundIncrement{0.1}
\newcommand\GroundSpacing{0.12}

\def\Ground#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \draw [line width=\WireLinewidth, color=WireColor]
        (\GroundWidth/2, 0) to (-\GroundWidth/2, 0);
    \draw [line width=\WireLinewidth, color=WireColor] 
        (\GroundWidth/2 - \GroundIncrement, -\GroundSpacing) to 
        (-\GroundWidth/2 + \GroundIncrement, -\GroundSpacing);
    \draw [line width=\WireLinewidth, color=WireColor]  
        (\GroundWidth/2 - 2*\GroundIncrement, -2*\GroundSpacing) to 
        (-\GroundWidth/2 + 2*\GroundIncrement, -2*\GroundSpacing);
\end{scope}
}

%%%%%%%%%%%%%%%%%%%
%% Inductor loop %%

\newcommand\LoopLength{2}
\newcommand\LoopWidth{1}

\def\Loop#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \coordinate (LR) at (-\LoopWidth/2, 0);
    \coordinate (CR) at (\LoopWidth/2, 0);
    
    \draw [line width=\WireLinewidth, color=WireColor, fill=Background, rounded corners=0] 
        ($ (LR) + (0, -\IndLength/2) $) to [out=180, in=-90, distance=\IndDistanceShort] 
        ($ (LR) + (-\IndWidth/2, -3*\IndLength/8) $) to [out=90, in=90, distance=\IndDistanceLong] 
        ($ (LR) + (+\IndWidth/2, -\IndLength/4) $) to [out=-90, in=-90, distance=\IndDistanceLong] 
        ($ (LR) + (-\IndWidth/2, -\IndLength/8) $) to [out=90, in=90, distance=\IndDistanceLong] 
        ($ (LR) + (+\IndWidth/2, 0) $) to [out=-90, in=-90, distance=\IndDistanceLong] 
        ($ (LR) + (-\IndWidth/2, \IndLength/8) $) to [out=90, in=90, distance=\IndDistanceLong] 
        ($ (LR) + (+\IndWidth/2, \IndLength/4) $) to [out=-90, in=-90, distance=\IndDistanceLong]
        ($ (LR) + (-\IndWidth/2, 3*\IndLength/8) $) to [out=90, in=180, distance=\IndDistanceShort] 
        ($ (LR) + (0, \IndLength/2) $) to [rounded corners=\WireCorners]
        ($ (LR) + (0, \LoopLength/2) $) to [rounded corners=\WireCorners]
        ($ (CR) + (0, \LoopLength/2) $) to [rounded corners=\WireCorners]
        ($ (CR) + (0, -\LoopLength/2) $) to [rounded corners=\WireCorners]
        ($ (LR) + (0, -\LoopLength/2) $) to [rounded corners=0] cycle;
\end{scope}
}
